Neural String Edit Distance

We propose the neural string edit distance model for string-pair matching and string transduction based on learnable string edit distance. We modify the original expectation-maximization learned edit distance algorithm into a differentiable loss function, allowing us to integrate it into a neural network providing a contextual representation of the input. We evaluate on cognate detection, transliteration, and grapheme-to-phoneme conversion, and show that we can trade off between performance and interpretability in a single framework. Using contextual representations, which are difficult to interpret, we match the performance of state-of-the-art string-pair matching models. Using static embeddings and a slightly different loss function, we force interpretability, at the expense of an accuracy drop.

==> table.tex <==
    \newcommand{\R}[2]{#1 \scalebox{0.8}}
    \resizebox{\textwidth}{!}{
    \centering\small
    \begin{tabular}{llccccccccccc}
        \toprule
        \multicolumn{2}{l}{\multirow{3}{*}{Method}} &
        \multirow{3}{*}{\rotatebox{90}{\# Param.}} &
            \multicolumn{5}{c}{Arabic $\rightarrow$ English} &
            \multicolumn{5}{c}{CMUDict}
            \\
            \cmidrule(lr){4-8} \cmidrule(lr){9-13}

        \multicolumn{2}{l}{}       &  &
            \multicolumn{2}{c}{Base} &
            \multicolumn{2}{c}{+ Int.\ loss} &
            \multirow{2}{*}{Time} &

            \multicolumn{2}{c}{Base} &
            \multicolumn{2}{c}{+ Int.\ loss} &
            \multirow{2}{*}{Time} \\
            \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){9-10} \cmidrule(lr){11-12}

        \multicolumn{2}{l}{}       &  & CER & WER & CER & WER &  & CER & WER & CER & WER & \\ \midrule

        \multicolumn{2}{l}{RNN Seq2seq} & 3.3M
                & \R{22.0}{0.2} & \R{75.8}{0.6} & --- & --- & 3.8m
                & \R{ 5.8}{0.1} & \R{23.6}{0.9} & --- & --- & 1.8h
                \\
        \multicolumn{2}{l}{Transformer} & 3.1M
                & \R{22.9}{0.2} & \R{78.5}{0.4} & --- & --- & 3.6m
                & \R{ 6.5}{0.1} & \R{26.6}{0.3} & --- & --- & 1.1h
                \\
        \midrule

        \multirow{5}{*}{\rotatebox{90}{ours}}
        & unigram          & 0.7M
                & \R{28.7}{1.2} & \R{84.5}{0.6} & \R{27.9}{0.5} & \R{85.3}{1.3} & 1.7h
                & \R{20.2}{1.1} & \R{64.4}{0.6} & \R{21.1}{0.6} & \R{67.5}{1.6} & 5.8h
                   \\
        & CNN (3-gram)     & ?
                   \\
        \cmidrule{2-13}
        & RNN              & 2.9M
                & \R{34.1}{3.4} & \R{88.1}{2.0} & \R{26.6}{1.2} & \R{81.4}{1.8} & 2.3h
                & \R{32.7}{9.2} & \R{80.2}{9.3} & \R{13.2}{1.2} & \R{52.5}{2.3} & 5.2h
                \\
        & \quad+ attention & 3.3M
                & \R{22.8}{0.3} & \R{76.9}{0.6} & \R{23.3}{0.5} & \R{77.6}{1.2} & 2.4h
                & \R{ 9.0}{0.4} & \R{36.6}{1.6} & \R{ 8.9}{0.6} & \R{36.4}{2.0} & 5.5h
                \\
        & Transformer      & 3.7M
                & \R{39.8}{9.1} & \R{91.1}{4.6} & \R{26.9}{0.7} & \R{83.3}{2.2} & 2.9h
                & \R{21.8}{0.4} & \R{70.6}{4.7} & \R{17.7}{1.0} & \R{61.2}{2.1} & 6.2h
                \\
        & \quad+ attention & 3.2M
                & \R{23.0}{0.5} & \R{77.0}{0.8} & \R{23.3}{0.3} & \R{78.0}{0.8} & 2.5h
                & \R{10.7}{0.3} & \R{42.3}{1.0} & \R{10.7}{0.3} & \R{42.9}{0.5} & 6.8h
                \\

        \bottomrule
    \end{tabular}}

